Demonstration-Guided Deep Reinforcement Learning of Control Policies for Dexterous Human-Robot Interaction

In this paper, we propose a method for training control policies for human-robot interactions such as handshakes or hand claps via Deep Reinforcement Learning. The policy controls a humanoid Shadow Dexterous Hand, attached to a robot arm. We propose a parameterizable multi-objective reward function that allows learning of a variety of interactions without changing the reward structure. The parameters of the reward function are estimated directly from motion capture data of human-human interactions in order to produce policies that are perceived as being natural and human-like by observers. We evaluate our method on three significantly different hand interactions: handshake, hand clap and finger touch. We provide detailed analysis of the proposed reward function and the resulting policies and conduct a large-scale user study, indicating that our policy produces natural looking motions.

==> RAL_handshake (copy)/sec/00_abstract.tex <==
% !TEX root = ../paper.tex

\begin{abstract}
In this paper, we propose a method for training control policies for human-robot interactions such as handshakes or hand claps via Deep Reinforcement Learning.
% 
The policy controls a humanoid Shadow Dexterous Hand, attached to a robot arm. 
%
We propose a parameterizable multi-objective reward function that allows learning of a variety of interactions without changing the reward structure. 
%
The parameters of the reward function are estimated directly from motion capture data of human-human interactions in order to produce policies that are perceived as being natural and human-like by observers. 
%
We evaluate our method on three significantly different hand interactions: handshake, hand clap and finger touch. 
%
We provide detailed analysis of the proposed reward function and the resulting policies and conduct a large-scale user study, indicating that our policy produces natural looking motions.
\end{abstract}

==> RAL_handshake (copy)/sec/01_introduction.tex <==
% !TEX root = ../paper.tex

\section{Introduction}


Dexterous humanoid hands, such as the Shadow Dexterous Hand \cite{shadowHand}, are becoming very sophisticated. Improvements in mechatronics have enabled very compact systems that have more than twenty degrees of freedom (DoF). However, controller design remains very challenging and has been shown to be a very complex problem \cite{rajeswaran2017learning, mordatch2012contact}. Recently, model-free deep reinforcement learning (DRL) algorithms have been applied to the control of humanoid hands, albeit on relatively simple tasks such as grasping or door opening \cite{rajeswaran2017learning} and in simulation only. %The results are demonstrated in only simulation. 
In \cite{openAI2018}, a controller trained in simulation has been transferred to a real humanoid hand. This opens up the door to learn policies for natural physical human-robot interactions. In particular, we are interested in learning a control policy for diverse hand interactions, such as handshakes or hand claps. The handshake is the most common greeting gesture throughout the world, therefore it has received a lot of attention in the robotics community \cite{knoop2017handshakiness, orefice2016let, arns2017design, shu2017learning, jindai2015handshake}. In this paper, we present a method for training a control policy for human-robot hand interactions, using data from human demonstrations in combination with deep reinforcement learning. We test our method on the simulated model of the Shadow Dexterous Hand.

% Forthermore, it has been shown that non-verbal communication and physical contact such as hugging are ... (comment: we can add this sentence)

%The importance of n
%It was show that non-verbal communication is more important than spoken language communication in terms of friendliness and liking \cite{argyle2013bodily}.

%Reaching similar DoF as the human hand enables robotic hands to reach human capabilities.

%Challenging problems are non-verbal interactions that involve physical contact, such as hugging \cite{block2018emotionally} or handshaking \cite{knoop2017handshakiness}.


%To achieve the long standing goal of having natural social interactions between humans and robots, researchers put emphasis on both verbal and non-verbal communication. It was show that non-verbal communication is more important than spoken language communication in terms of friendliness and liking \cite{argyle2013bodily}. Challenging problems are non-verbal interactions that involve physical contact, such as hugging \cite{block2018emotionally} or handshaking \cite{knoop2017handshakiness}. Handshake is the most common grating gesture throughout the world, therefore it received a lot of research attention in the robotics community \cite{knoop2017handshakiness, orefice2016let, arns2017design, shu2017learning, jindai2015handshake}. However, humans are performing different forms of hand interactions such as high fives, fist bumps, holding hands etc. With the development of dexterous humanoid hands, these interactions can be also executed by a humanoid robot. In this paper, we explore the possibility of preforming different forms of hand interactions between a human and a robot. As a test platform, we use the simulated model of a Shadow dexterous hand \cite{shadowHand}. 

%Dexterous humanoid hands, such as the Shadow hand, have been available on the market for several years. Improvements in mechatronics enabled very compact systems that have more than twenty degrees of freedom (DoF). Reaching similar DoF as the human hand enables robotic hands to reach human capabilities. Furthermore, humanoid hands appear very natural to humans, which makes them an ideal platform for human-robot interactions, especially in cases which involve hand interactions. To use humanoid hands, the main challenge is to design a controller, which is shown to be a very complex problem \cite{rajeswaran2017learning, mordatch2012contact}. Recently, few model-free deep reinforcement learning (DRL) algorithms are applied to a control problem of humanoid hands. \cite{rajeswaran2017learning} shows remarkable performance in a simulation on standard tasks such as grasping or door opening. In \cite{openAI2018}, it was shown that the controller trained in a simulation can be transferred from the simulation to a real platform. We therefore follow the model-free DRL approach.  

%To train a control policy using a DRL algorithm, one of the main issues is the definition of a reward function. For a lot of tasks, the goal is obvious and the reward can thus be shaped to reach this goal \cite{rajeswaran2017learning}. For our task, however, specifying a reward function is not obvious. The goal of the robot is to perform an interaction \emph{and} to produce natural motions and contacts. Thus, there are multiple objectives that need to be considered in order to perform a successful interaction. If implemented naively, each interaction would require a specialized reward function because hand poses and contact profiles are different. Therefore, we propose a generalized reward function that takes multiple objectives, such as contact patterns and goal positions, into account and works across different interaction types. The parameters of the reward function are extracted automatically from motion capture data of human hand interactions.
%Another issue is setting up the training algorithm in order to achieve the best convergence properties. Standard DRL algorithms, e.g., DDPG \cite{lillicrap2015continuous}, work out of the box on benchmark problems \cite{openAiGym}. However, for more complex problems, additional training components need to be added, such as early stopping \cite{peng2018deepmimic} or using human demonstrations \cite{vecerik2017leveraging, rajeswaran2017learning}. We propose a training algorithm which works in combination with DDPG.

To train a control policy using a DRL algorithm, one of the main issues is the definition of a reward function. For simple tasks, like grasping or pick and place tasks, the goal is obvious and the reward can be easily shaped. For our task, however, it is not obvious how to shape a reward function. The reward needs to result in motions that are perceived as natural, the hand needs to reach a desired contact profile and precise position, while dealing with complex contact dynamics.
%, while dealing complex contact dynamics.
%Reward shaping is challenging for two main reasons. First, the the hand motion needs to look natural. Second, the robot hand needs to be precisely positioned with respect to the other hand while dealing with complex contact dynamics.
%the robot hand needs to coordinate its motions with respect to the other hand and deal with complex contact dynamics. 
%\Stefan{Second, the hand motion is executed in the presence of contact with the other hand, and contacts are uncertain.}
%The policy needs to overcome two main challenges, the first is that the motion looks natural and second is to achieve the first goal in presence of motions and contact with the other hand. 
To produce natural looking motions of animated characters in \cite{peng2018deepmimic}, the reward  is based on tracking position and angle references from motion capture data. However, the authors only consider motions in open space and hence their reward function cannot be transfered to our task. 
Thus, we investigate important terms to construct a reward function and compare the influence of different reward terms in an ablation study.  
%The standard approaches for generating natural motions, such as \cite{peng2018deepmimic}, only consider motions in open space. Thus, the reward function is based solely on tracking joint positions and angles obtained from motion capture data, which does not produce satisfying results for hand interaction tasks. 
%We investigate what are the important terms to construct a parametrized reward function and show how each of the terms contribute to the main result in the ablation study.
%Therefore, we come up with a parametrized reward function.
%We define the most important reward ingredients and show how each of the ingredients contribute to the main result in the ablation study. 
%We demonstrate that our reward function can be used to learn diverse hand interactions in RL framework.
To enable generalization to different hand interactions, we define a parametrized reward function. %with multiple open parameters. 
%As usually done when the goal is to generate natural motions, 
We extract most of the reward function parameters from motion capture data, leading to only six parameters that are relatively easy to adjust. 
One could argue that the policy could be learned directly from data via Inverse Reinforcement Learning (IRL). However, state-of-the-art IRL methods \cite{ho2016generative, merel2017learning} have not been applied to tasks that require precise positioning or challenging contact dynamics. Furthermore, these methods can be unstable when applied to motion capture data \cite{merel2017learning}.  
%However, our task requires precise positioning which is still not demonstrated with IRL methods. Furthermore, state-of-the-art methods can be very unstable when working on motion capture data \cite{merel2017learning}.   
%However, state-of-the-art methods can be very unstable, when applied to tasks of similar complexity \cite{merel2017learning}. 
%Thus, manually designed reward functions \cite{peng2018deepmimic} are still preferred. 
To ensure training convergence, we propose a specialized training method. Standard DRL algorithms work out of the box on benchmark problems \cite{openAiGym}, but for more complex problems additional training details, such as randomization or early stopping are important \cite{peng2018deepmimic, vecerik2017leveraging, rajeswaran2017learning}.
We propose a training method which works in combination with DDPG, resulting in stable convergence properties.

%However, for more complex problems, additional training components need to be added, such as early stopping \cite{peng2018deepmimic} or using human demonstrations \cite{vecerik2017leveraging, rajeswaran2017learning}. 


%To train a control policy using a DRL algorithm, one of the main issues is the definition of a reward function. For simple tasks, like grasping or pick and place tasks, the goal is obvious and the reward can be easily shaped. For our task, however, it is not obvious how to shape a reward function. The reward needs to result in motions that are perceived as natural and the hand needs to reach precise position, while dealing complex contact dynamics. To produce natural looking motions in \cite{peng2018deepmimic}, the reward function is based on tracking position and angle references from motion capture data. However, the authors only consider motions in open space and their reward function cannot be transfered to our task. Thus, we investigate what are the important terms to construct a reward function and compare influence of different reward terms in the ablation study. To enable generalization to different hand interactions, we define a parametrized reward function with multiple open parameters. As commonly done when goal is to generate natural motions, we extract the parameters from motion capture data, leading to only six parameters that are relatively easy to adjust. Alternatively, one could argue that policy can be learned directly from data. However, state-of-the-art methods can be very unstable, when applied to tasks of similar complexity \cite{merel2017learning}. Thus, manually designed reward functions \cite{peng2018deepmimic} are still preferred. Finally, to ensure the training convergence we develop a training method. Standard DRL algorithms work out of the box on benchmark problems \cite{openAiGym}. However, for more complex problems, additional training components need to be added, such as early stopping \cite{peng2018deepmimic} or using human demonstrations \cite{vecerik2017leveraging, rajeswaran2017learning}. We propose a training method which works in combination with DDPG, that results in stable convergence properties.

%Our parametrized reward function relies on motion capture data to obtain the parameters. The reward function is designed to work for different hand interactions, which results in relatively large number of open parameters. We automatically extract the parameters of the reward function from the motion capture data, leading only to 6 parameters that are relatively easy to tune. 

 %and thus can be used to generate different hand interaction policies. 




%We define a parametrized reward function which can be used to generate different hand interaction policies. 


%Our reward function is parametrized to work 

%To produce natural looking motions, the natural choice is to base the reward function on motion capture data. 


%To produce natural motions, we base our reward function on motion capture data. Our reward function has multiple parameters which cannot be tuned easily by hand. It is hard to design reward function with few parameters that works for all interactions.
%Since our goal is to produce natural looking motions, the reward function should be based on real hand interaction data \Stefan{maybe to emphasize better why is beneficial to extract parameters from data.}.
%\Stefan{Since our goal is to produce natural motions, we want to extract the parameters of the reward function from the motion capture data, as usually done.} 
%We automatically extract the parameters of the reward function from the motion capture data, leading only to 6 parameters that are relatively easy to tune. 

%In contrast, one could ask, why we do not learn the reward function from scratch using the given data. For tasks of similar complexity, methods such as \cite{merel2017learning} were used to train the policy directly from data. However, these methods tend to be very unstable, thus for complex task manually designed reward functions \cite{peng2018deepmimic} are still preferred . DRL is a powerful policy learning framework. Standard DRL algorithms work out of the box on benchmark problems \cite{openAiGym}. However, for more complex problems, additional training components need to be added, such as early stopping \cite{peng2018deepmimic} or using human demonstrations \cite{vecerik2017leveraging, rajeswaran2017learning}. We propose a training method which works in combination with DDPG, that results in stable convergence properties \Stefan{(and robustness)}. 


%, thus a single cost function that works over different hand interactions would be desirable

%\Stefan{(comment: for second problem, we need to specify what we solve. this is still open)}

%Furthermore, for arbitrary interaction types, our goal is to use the same reward function. Ideally, we would like to extract the reward directly from data which contains human interaction sequences. In this paper, we generate the reward function automatically from the motion capture data of human hand interactions.    


%is training procedure of the of the DRL algorithm. Although the reward function can produce good results, the resulting policy might not converge to the desired solution in some cases, or converges very slowly. Furthermore, the policy might not be robust to the environment perturbations. To resolve these issues, we apply a specific training procedure. 

\begin{figure}
\centering
	\includegraphics[width= 0.85 \linewidth]{figures/first_fig_2.png}
	\caption{\small{Approach overview. The proposed multi-objective reward function and extracted parameters from human interaction data are used to train a human-robot interaction control policy via DRL.}}
	\label{fig:first_figure}
\end{figure}

This work presents a method for learning control policies for dexterous human-robot interaction. More specifically, we contribute the following:
\begin{inparaenum}[(i)]
	\item A multi-objective reward function for DRL algorithms. We show how reward function parameters are extracted from motion capture data and provide detailed analysis of how different parts of the reward influence the resulting control policy. %The function works for various gestures with only few varying parameters.
	\item A training method which works in combination with standard DRL algorithms.
	\item A dataset of human hand interactions. % and the data collection procedure.
	\item A large-scale user study showing that adding imitation reward to the policy results in motions that are perceived as more natural. 
\end{inparaenum}

 



==> RAL_handshake (copy)/sec/02_related_work.tex <==
% !TEX root = ../paper.tex

\section{Related Work}

\subsection{Human Hand Interaction}

Different aspects of the human-robot handshake problem were investigated in the robotics community, e.g., force properties of a human handshake \cite{knoop2017handshakiness}, the possibility to recognize personality and gender from a handshake \cite{orefice2016let}, or the design of a compliant controller for handshakes \cite{arns2017design}.
Previous work mostly focuses on the handshake properties after the contact phase. However, producing a handshake movement is equally important \cite{shu2017learning, jindai2015handshake}. When humans establish a handshake, one person requests the handshake by holding out one hand, while the other person responds by grabbing the hand \cite{jindai2015handshake}. Based on this observation, \cite{jindai2015handshake} tries to model the appropriate time to request a handshake.

%In \cite{jindai2015handshake}, the model for making a handshake request motion was investigated. 
%They create this model using motion capture data of human handshake motions.

%The problem of handshaking with a robot was investigated from various aspects in the robotics community \cite{knoop2017handshakiness, orefice2016let, arns2017design}.
%In \cite{knoop2017handshakiness}, the authors investigate force properties of a human handshake, i.e., where pressure is applied and what the range applied forces is. Researchers also investigated the possibilities to recognize human personality and gender from the handshake \cite{orefice2016let}. \cite{arns2017design} shows the design of a compliant controller in order to perform a handshake. 

To achieve a handshake with humanoid hands, usually the robot requests the handshake and closes the fingers when the human hand is in contact \cite{arns2017design}. To the best of our knowledge, our method is the first that treats the problem in the case where the human requests the handshake. This case is harder from a control perspective, because it requires coordination with the human hand, the robot needs to produce natural looking motions and it still involves physical contact as in the previous case. The control of robotic arm movement is investigated in \cite{shu2017learning, jindai2015handshake}, but these papers do not control humanoid hands and do not observe complex contact dynamics. Furthermore, we investigate the possibility of performing different hand interactions, such as hand claps or finger touches, which are relatively under-researched.

% In \cite{calinon2007incremental}, the robot learns to perform different gestures, but none of these gestures involve physical contact.

\subsection{Control of Dexterous Humanoid Hands}

Dexterous humanoid hands are a highly complex mechanical systems \cite{kumar2013fast}. Due to their high complexity, the control problem is shown to be very challenging \cite{rajeswaran2017learning, mordatch2012contact}. Most approaches therefore use trajectory optimization to provide a controller \cite{mordatch2012contact, bai2014dexterous, kumar2014real}. These approaches require a precise model of the system, which makes them hard to transfer to real robots.
Leveraging real robot data for model learning was proposed in \cite{kumar2016optimal}, but the method is limited to slow in-hand manipulation of a pole. Contrary, model-free DRL does not require a model of the robot dynamics, i.e., all information is obtained through multiple episodes of trial-and-error. The only input to the algorithm is a reward function. Recently, model-free DRL has been applied to the control problem of humanoid hands \cite{rajeswaran2017learning},  achieving impressive results in a simulated environment. Furthermore, \cite{openAI2018} demonstrates the possibility of transferring a policy trained in simulation to the real Shadow Dexterous Hand. 

%In our work, we therefore use model-free DRL, since it can achieve high performance policies and offers the possibility to learn from human demonstrations. 


For non-linear control tasks, model-free DRL algorithms have shown impressive performance \cite{lillicrap2015continuous, schulman2015trust, schulman2017proximal} on the OpenAI gym benchmark problems \cite{openAiGym}. Furthermore, when applied to low degree of freedom robotic manipulators (7-10 DoF), like robotic hands with grippers, model-free DRL has been leveraged successfully \cite{gu2017deep, vecerik2017leveraging, rusu2017sim}. However, the problem becomes more challenging when DRL is applied to systems with higher DoF. A hand control problem \cite{rajeswaran2017learning} or natural movement character control problem \cite{peng2018deepmimic} deal with such systems. 
In \cite{peng2018deepmimic}, the authors carefully design and adjust the weights of the reward to achieve the desired performance. 
To improve convergence properties, the authors use two training techniques: setting the initial state on the demonstration trajectory and early stopping. 
Human demonstration can be used to accelerate the convergence rate \cite{rajeswaran2017learning}. In \cite{rajeswaran2017learning}, a human operator provides demonstrations via teleoperation, which are used to initialize the policy. 
Alternatively, IRL methods \cite{abbeel2004apprenticeship, ziebart2008maximum, wulfmeier2015maximum} can learn the reward function from demonstration data. However, they require running the RL algorithm in the inner loop of an iterative method, which is not feasible with DRL algorithms. To overcome this issue, IRL is posed as an adversarial imitation problem \cite{merel2017learning, ho2016generative}, but these methods are prone to instability.

%but they require running RL algorithm in the inner loop of an iterative method. This is not feasible with the DRL algorithm in the inner loop. Thus, IRL is posed as adversarial imitation problem \cite{merel2017learning, ho2016generative} to work with DRL methods, but these methods are unstable especially in presence of noisy motion capture data.


%Inverse reinforcement learning REF learns the cost function directly from data. These methods require RL method in training loop which for current task is infisable because of computation time. Methods that successfully learn motion tasks from data are adversarial imitation leaning methods. However, they can be unstable \cite{merel2017learning}, which is even more problematic whit noisy motion capture data for precise tasks such as ours.

%\Stefan{Alternatively, one could use adversarial imitation leaning from motion capture data, but this can be unstable \cite{merel2017learning}.}

%Model-free DRL does not require a model of the robot dynamics, i.e., all information is obtained through multiple episodes of trial-and-error. The only input to the algorithm is a reward function. However, it is not straightforward to make these algorithms work on real world problems. Although it has been shown that transfer from a simulation to the real robot is possible \cite{tobin2017domain, rusu2017sim, peng2017sim}, making the algorithm work even in the simulation can be challenging. 

%When applied to low degree of freedom robotic manipulators (7-10 DoF), like robotic hands with grippers, model-free DRL has achieved a lot of success \cite{gu2017deep, vecerik2017leveraging, rusu2017sim}. However, for systems with higher DoF, such as hand control \cite{rajeswaran2017learning} or character animation \cite{peng2018deepmimic}, the problem becomes more challenging. In \cite{peng2018deepmimic}, the authors need to carefully design and adjust the weights of the reward function to achieve a high level of performance. To improve convergence properties, the authors use two techniques in training: setting the initial state on the demonstration trajectory and early stopping. Human demonstration can be used to accelerate the convergence rate \cite{rajeswaran2017learning}. In \cite{rajeswaran2017learning}, a human operator provides demonstrations via teleoperation, which is used to initialize the policy. 

%Model-free deep reinforcement learning (DRL) was applied to low degree of freedom robotic manipulators (7-10 DoF), like robotic hands with grippers, with a lot of success \cite{gu2017deep, vecerik2017leveraging, rusu2017sim}. 
%The large number of training samples required and safety reasons are still major barriers for these algorithms to be applied on the real robot. However, it was shown that polices trained in a simulation can be transfered to the real robot \cite{tobin2017domain, rusu2017sim, peng2017sim}.

Our method is inspired by previous DRL approaches, but our task requires significant changes of existing methods. In \cite{rajeswaran2017learning}, the demonstrations are provided by teleoperating a simulated robot hand, operating in isolation. 
For our case, it is impractical to collect demonstrations this way because it requires interactions between two humans. Thus, we capture real interactions using a motion capture system. %Also, correct contact patterns are not a direct objective and are therefore not considered in the reward. 
%Furthermore, the hand is attached to the robot arm in our system, which makes teleoperation much harder. MAYBE TO RETURN
Our method is more similar to \cite{peng2018deepmimic}, which is not designed for humanoid hands. 
In \cite{peng2018deepmimic}, the authors use motion capture data directly in the reward function formulation. Contrary, we extract the final pose parameters from data, while we similarly use motion capture data to produce natural looking motions. Additionally, we add contact patterns as an objective to the reward function, and provide a different training method.  
%The training techniques from \cite{peng2018deepmimic} are not applicable to our case. Thus, we provide a training method that produces hand interaction policies.
 

% Contrary, we extract the final reward function parameters directly from data, while we still leverage data to produce natural looking motions.  
 


%Alternatively, inverse reinforcement learning methods, such as \cite{ho2016generative}, can be used to learn the reward function, but it has been shown that they require long training times and can have unstable convergence properties.   

%However, they iteratively shape the reward function by running DRL training in each iteration, which would results in extremely long training times.

%\Stefan{(comment: What do we do, how we are different? - we design cost from mocap, we use imitation but also start from random pose).} 
%\Stefan{(comment: This whole subsection needs to be revisited. Needs to separate stuff and make them in right order).} 

% Downside of \cite{rajeswaran2017learning} it that requires significant amount of human demonstrations provided via teleoperation in the simulation environment. Since we need to record interaction between two humans, it is impractical to collect demonstrations in the simulation environment. We collect interaction demonstrations using motion capture system. Furthermore, in \cite{rajeswaran2017learning} the hand is controlled via teleoperation while floating in the air. In our environment, the humanoid hand is attached to a robot arm, which makes the teleoperation task much harder.
 
%\Stefan{comment: Our method is mostly focused on cost design, so I do not know do we need to argue so much about clasical methods. Probably imitation is very hard to do with old methods. DRL offers more flexibility. Probably the best argument is to say something like DRL outperforms old methods and offers more flexibility thats why we use these methods. }


%\subsection{Model-free Deep Reinforcement Learning}

%In the last few years, model-free deep reinforcement learning (DRL) managed to solve complicated decision making problems. It achieved human level performance in playing Atari games \cite{mnih2013playing} and managed to solve complex continuous control problems \cite{lillicrap2015continuous, schulman2015trust, schulman2017proximal}.  

%Most of the results of model-free DRL algorithms are obtained in simulation. The large number of training samples required and safety reasons are still major barriers for these algorithms to be applied on the real robot. Only recently, few approaches enable model-free DRL algorithms to be applied on real robots. These approaches either use transfer learning \cite{openAI2018, tobin2017domain, peng2017sim} to transfer a policy trained in the simulation to the real robot, or human demonstration to reduce training time \cite{vecerik2017leveraging}. For humanoid hands, \cite{openAI2018} shows remarkable results, which gives promises that transfer from the simulation to the real robot is possible even in case with highly complex dynamics of the robot.  

==> RAL_handshake (copy)/sec/03_preliminaries.tex <==
% !TEX root = ../paper.tex

\section{Preliminaries}

\subsection{Deep Reinforcement Learning}
\label{sec:drl}

\newcommand{\StatesSet}{\mathcal{S}}
\newcommand{\ActionsSet}{\mathcal{A}}
\newcommand{\TransitionSet}{\mathcal{T}}
\newcommand{\state}[1]{{s}_{#1}}
\newcommand{\action}[1]{{a}_{#1}}
\newcommand{\reward}{r}
\newcommand{\discountRate}{\gamma}
\newcommand{\QFunction}{Q}
\newcommand{\policy}{\pi}
\newcommand{\Cost}{J}
\newcommand{\mdp}{\mathcal{M}}


Our control problem can be formalized using Markov Decision Processes (MDP), defined as a tuple $\mdp = \{\StatesSet, \ActionsSet, \mathcal{R}, \mathcal{T}, \rho_0, \discountRate \}$. We describe an environment with a set of states $\StatesSet$, a set of actions $\ActionsSet$, a reward function $\mathcal{R} = \reward(\state{t}, \action{t})$, transition dynamics $\mathcal{T} = p(\state{t+1}|\state{t}, \action{t})$, an initial state distribution $\rho_0 = p(\state{1})$ and a discount rate $\discountRate \in [0,1]$, where $\state{t} \in \StatesSet$ and $\action{t} \in \ActionsSet$. Model-free RL does not require knowledge of transition dynamics and requires only sampling from the transition dynamics probability distribution.  
We define the return $R_{t}$ as a discounted sum of future rewards:
\begin{equation}
R_{t} = \sum_{i=t}^{T}\discountRate^{i-t}\reward(\state{i}, \action{i}).
\end{equation}
The controller is defined as a control policy $\policy$, which maps states to actions $\policy: \StatesSet \rightarrow \ActionsSet$. The goal of the reinforcement learning algorithm is to learn a policy $\policy$ which maximizes the expected return from the start distribution:
\begin{equation}
\Cost = \mathbb{E}_{\mdp} \left [R_{1} \right ]
\end{equation}

We define the action-value or Q-function, which describes the expected return under a policy $\policy$ when taking action $\action{t}$ from state $\state{t}$, also called state-action pair, as follows: 
\begin{equation}
Q(\state{t}, \action{t}) = \mathbb{E}_{\mdp} \left [ R_{t}  \middle\vert \state{t}, \action{t} \right ].
\end{equation}

To solve the given problem, we define the Q-function and policy as neural network function approximators parametrized with $\theta^Q$ and $\theta^{\policy}$. This is known as an actor-critic type of RL algorithm, since we learn both an actor function, i.e., the policy, and a critic function, i.e., the Q-function. More specifically, we use the DDPG algorithm \cite{lillicrap2015continuous} to compute the gradients for updating the neural network parameters. To update  $\theta^Q$, we minimize the loss:
\begin{align}
&L(\theta^Q) = \mathbb{E}_{\mdp, \action{t}} \left [ \left( Q(\state{t}, \action{t} ; \theta^Q) - y_t \right)^2   \right] \\
&y_t = \reward(\state{t}, \action{t}) + \discountRate Q(\state{t+1}, \action{t+1} ; \theta^Q) 
\end{align} 
To update the actor parameters $\theta^{\policy}$, we compute the gradients:
\begin{equation}
\nabla_{\theta^{\policy}} \Cost = \mathbb{E}_{\mdp} \left [\nabla_{\theta^{\policy}} Q(\state{t}, \action{t} ; \theta^Q)    \vert \state{t}, \action{t} = \policy(\state{t} ; \theta^{\policy}) \right ],
\end{equation}
which are applied to the actor neural network. For both networks we use three fully connected layers with $256$ neurons and ReLu activation functions.

To ensure convergence of the policy, we apply all techniques from the DDPG paper to stabilize convergence properties. This includes a replay buffer, batch normalization and target networks. DDPG is an off-policy algorithm, thus we define the exploration policy as:
\begin{equation}
\action{t} = \policy(\state{t}) + \mathcal{N}, 
\end{equation}
where $\mathcal{N}$ is a sample from zero mean Normal distribution. More implementation details can be found in \cite{lillicrap2015continuous}.

%To define the relationship between a state-action pair $(s,a)$ and successive state-action pairs $(s',a')$ recursively, we can rewrite this equation as follows:
%\begin{equation}
%Q_{\pi}(s,a) = \sum_{a}\pi(a|s)\sum_{s',r}p(s',r|s,a)[r+\gamma\text{ }%Q_{\pi}(s',a')],
%\end{equation}
%which is called the Bellman equation.

%The goal of the agent is to maximize the expected reward, i.e., to know the optimal action to take at a specific state and timestep in order to gain maximum reward in the long run. More formally, we introduce a discount rate $\discountRate \in [0,1]$ and the sum of future rewards, which we call return: 
%\begin{equation}
%R_{t}\doteq \sum_{i=t}^{T}\gamma^{i-t}r_{i},
%\end{equation}
%where T marks the termination step of an episode. \Stefan{switch to infinity case}. Given an initial state $s_{0}$ of an episode, the goal of the agent is to maximize the expected return $\mathbb{E} [R_{1}|s_{0}]$, i.e., to find a policy which selects the actions that will maximize the expected return.


\subsection{Simulation Environment}

\begin{figure}
\centering
	\includegraphics[scale=0.17]{figures/arm_and_hand_cropped.png}
	\caption{\small{Agent arm with the Shadow Dexterous Hand. The system has 28 DoF. The arm, shown in blue in the left figure, has 4 Dof. The hand has 24 Dof, depicted as yellow cylinders in the right figure, and 20 actuators. Contact sensors are marked in purple (right).}}
	%\vspace{-0.5cm}
	\label{fig:dof}
\end{figure}

Our simulation environment consist of two robots: the agent, controlled by the policy, and the target hand. The agent consists of a 4 DoF robotic arm and the Shadow Dexterous Hand with 24 DoF. The Shadow Dexterous Hand is controlled by 20 actuators (cf. Fig.~\ref{fig:dof}). We use the same hand model as stand-in for a human hand for convenience, since this model is easy to pose in different configurations. However, this model can be replaced with a human hand model, which should not influence the results of our experiments since the hand is not actuated, as usually assumed for a hand requesting an interaction \cite{shu2017learning, jindai2015handshake}. The robot models are taken from the OpenAI gym framework \cite{openAiGym}. %, whereas our environment is custom made. 


The input to the control policy are joint angles, joint velocities and contact sensor readings (cf. Fig.~\ref{fig:dof}) of the agent hand. Additional inputs are the positions of the target hand links and the origin of each rigid body on the hand. The policy outputs are control signals that actuate the agent's arm and hand. Control signals are setpoints for the joint angles scaled in the range from $-1.0$ to $1.0$. %, as is the default in the OpenAI gym for robotic arms and hands.

==> RAL_handshake (copy)/sec/04_method.tex <==
% !TEX root = ../paper.tex

\section{Method}

Our method is able to learn control policies of hand interactions using motion capture data of human demonstrations. We assume the following setting: the first participant requests the interaction while the second is executing the interaction sequence. In the example of a handshake, the first participant stretches out the hand to request the handshake, while the other responds by grabbing the hand. The robot learns to perform the behavior of the second participant. The goal is to produce the desired interaction \emph{and} motions perceived as natural. 
We propose a \emph{single} reward function that can be applied to various hand interactions. 
%\Stefan{Contributions of each reward term to the final policy are explained throughout Sec.~\ref{sec:rew_func}.} 
The parameters of the reward function are extracted directly from the motion capture dataset using Alg.~\ref{alg:1}. The policy is trained via a DDPG based training method, as explained in Sec.~\ref{sec:training_alg}.

%and describe the system for collecting 

%We developed a training algorithm which uses DDPG in order to train hand interaction policies. Additionally, we provide a method for collecting motion capture data of human interactions. 

\newcommand{\gain}{\omega}
\newcommand{\dataset}{\mathcal{D}}
\newcommand{\indicator}{\mathds{1}^i_{ct}}
%\newcommand{\indicator}{1^c_i}

\subsection{Reward Function}
\label{sec:rew_func}


Our proposed reward function consists of two terms:
\begin{equation}
\reward(\state{t}, \action{t}) = \reward_F(\state{t}, \action{t}) + \reward_I(\state{t}, \action{t}),
\end{equation}
where $\reward_F(\state{t}, \action{t})$ is the final state reward, which is used to reward the correct end configuration, and  the imitation state reward $\reward_I(\state{t}, \action{t})$, which provides trajectory guidance to make the interactions look more natural.
%
The final state reward itself consists of four terms:
\begin{equation}
\reward_F(\state{t}, \action{t}) = \reward_p(\state{t}) + \reward_{\alpha}(\state{t}) + \reward_c(\state{t}) + \reward_a(\action{t}),
\end{equation}
where $\reward_p(\state{t})$ is a position reward, $\reward_\alpha(\state{t})$ is an angle reward, $\reward_c(\state{t})$ is a contact reward, and $\reward_a(\action{t})$ penalizes high action inputs. Experimentally, we determined that the most important position features are the fingertip positions of the agent hand (total number $N_f = 5$). Regarding the angles, we use all joint angles of the robot hand to compute the angle reward (total number $N_{\alpha} = 24$). Position and angle rewards are defined as a negative $l_2$ norm of position features and angle errors:
\begin{align}
& \reward_p(\state{t}) = - \sum_{i=1}^{N_f} \omega^i_p  \vert\vert p^i_g - p^i_{rt} \vert \vert \\
& \reward_{\alpha}(\state{t}) = - \sum_{i=1}^{N_{\alpha}} \omega^i_{\alpha} \vert\vert \alpha^i_g - \alpha^i_{rt} \vert\vert.
\end{align}
The vector $p^i_g$ is the goal position of each position feature and $p^i_{rt}$ is the current position of the respective feature. Similarly, $\alpha^i_g$ is the goal joint angle and $\alpha^i_{rt}$ the current joint angle on the robot hand. The weights $\omega^i_p$, $\omega^i_{\alpha}$ determine the importance of the specific goal, which we define via algorithm described in Sec.~\ref{sec:reward_alg}. When using only position and angle rewards, the robot hand only roughly reaches the desired end configuration (cf. Fig~\ref{fig:experiment_1_poses}, Baseline 2). 
Our task requires accurate hand positioning, which is hard to achieve in tasks that involve contacts.
We achieve the desired hand position by adding a contact reward $\reward_c(\state{t})$, which forces the desired contact profile.
%The combination of position, angle and contact rewards results in the most accurate end configuration. 
For more details about the influence of the reward terms we refer to Sec.~\ref{sec:abl_study}.
Additionally, a control input reward is added to prevent high control signals. Contact and input rewards are defined as:
\begin{align}
& \reward_c(\state{t}) = \sum_{i=1}^{N_{c}} \gain^i_c \indicator \quad ,\\
& \reward_a(\action{t}) = - \sum_{i=1}^{N_{a}} \gain^i_a  \vert\vert a^i \vert\vert^2 \quad ,
\end{align}
where the indicator function $\indicator$ outputs $1$ in case the contact sensor is active and $0$ otherwise. The weight $\gain^i_c$ determines the importance of each contact sensor. The system has $N_{c} = 15$ contact sensors. $a^i$ is the control input signal for each actuator and $\gain^i_a$ is the respective weight. The system has $N_a = 24$ control inputs.

%When using only position and angle rewards, the robot hand can only roughly reach the desired pose (cf. Fig~\ref{fig:experiment_1_poses}). To achieve the desired goal pose, we add contact reward $\reward_c(\state{t})$. In presence of contacts, achieving precise hand pose is very hard relying only on the position based reward.
%This is a crucial difference compared prior work REF, which usually use only position and angle information. 
%We argue, that combination of position and angle rewards with the contact reward produces \Stefan{more natural hand poses}. For more details about the reward terms, refer to Sec.~\ref{sec:abl_study}


The imitation reward consist of two further terms:
\begin{equation}
\reward_I(\state{t}, \action{t}) = \reward_{p I}(\state{t}) + \reward_{\alpha I}(\state{t}).
\end{equation}
The difference compared to the final state reward is that the goal position $p^i_{g t}$ and goal angles $\alpha^i_{g t}$ depend on the timestep:
\begin{align}
& \reward_{p I}(\state{t}) = - K_{p I} \sum_{i=1}^{N_f} \omega^i_{p} \vert \vert p^i_{g t} - p^i_r \vert \vert \quad ,\\
& \reward_{\alpha I}(\state{t}) = - K_{\alpha I} \sum_{i=1}^{N_{\alpha}} \omega^i_{\alpha} \vert\vert \alpha^i_{gt} - \alpha^i_r \vert\vert.
\end{align}
These rewards are scaled with the weights $K_{p I}$ and $K_{\alpha I}$.

%Reward function that uses only final state reward results in a correct end pose, but the approaching trajectory can look unnatural, as shown Sec.~\ref{sec:imitation_eval}. Therefore, we add imitation reward to produce more natural hand motions.

The final state reward function is often enough to complete the interaction, i.e., to reach the final pose. However, the most direct trajectory often does not look natural (cf. Fig.~\ref{fig:experiment_2_qual_clap}). 
%\Stefan{For example, in the case of a hand clap, the agent would simply position its hand on the target hand, omitting the characteristic clapping motion entirely.} 
We overcome this issue by adding an imitation reward. As shown in Sec.~\ref{sec:imitation_eval}, imitation reward significantly improves that the hand motion is perceived as natural.
However, when the starting hand pose is far away from poses in demonstration examples, the policy may produce non-smooth motions. We evaluate these examples also in Sec.~\ref{sec:imitation_eval}.

 

\subsubsection{Reward function parameters}
\label{sec:reward_alg}
To define the terms of the reward function, we use a  motion capture dataset $\dataset = \{(p^{i}_{t}, p^{j}_{t}, \alpha^{i}_t, \alpha^{j}_t) \}_{t=1}^T$ of an interaction sequence. The dataset provides positions of rigid bodies $p^{i}_{t}, p^{j}_{t}$ and joint angles $\alpha^{i}_t, \alpha^{j}_t$ of two human hand models at timestep $t$: the target hand, denoted with superscript $j$, which requests the interaction and the actor hand, denoted with superscript $i$, which the robot imitates. From $\dataset$, we can calculate distances between the rigid bodies $d^{ij}_t$ and the relative position calculated in the coordinate frame of the target hand body $\Delta  p^{ij}_t$. 
We use fingertip positions on both hands, plus the palm position on the target hand. For the joint angles, we use all joints from the human data that have a corresponding joint on the robot hand. Based on the minimum distance, we set the reference frame $j_{\min}$ and reference timestep $t_{\min}$, as shown in Alg.~\ref{alg:1}.  Using these references, we compute the goal positions and goal angles. 
%
The position goals are defined in a goal centric way, which enables us to calculate them for a randomly positioned hand in the simulation $ p^j_{s}$, as shown in line 5 of Alg.~\ref{alg:1}, where $R^j_s$ is the rotation matrix of the target hand rigid body with index $j$.
\begin{algorithm}
\caption{Reward Parameters}\label{alg:1}
\begin{algorithmic}[1]
\State \textbf{Input:} $\dataset, d^{ij}_t, \Delta  p^{ij}_t$ 
\State $t_{\min} \gets \arg\min d^{ij}_t$, \quad $j_{\min} \gets \arg\min d^{ij}_t$
\State $p_s^{j_{\min}} \gets$ position of a $j_{\min}$ link in simulation 
\State $R_s^{j_{\min}} \gets$ rotation matrix of a $j_{\min}$ link in simulation
\State $p^i_g \gets p^{j_{\min}}_s + R^{j_{\min}}_s \Delta p_{t_{\min}}^{ij_{\min}}$,  \quad $\alpha^i_g \gets \alpha_{t_{\min}}^i$
\State $p_{g t}^i \gets p_s^{j_{\min}} + R_s^{j_{\min}} \Delta p_{t}^{ij_{\min}}$,  \quad $\alpha_{g t}^i \gets \alpha_{t}^i$
\State \Return $p_g^i,\alpha_g^i, \{\alpha_{g t}^i \vert t=1..t_{\min} \}, \{p_{g t}^i \vert t=1..t_{\min} \} $
\end{algorithmic}
\end{algorithm}

%We find the minimum distance between the key hand positions to set the reference frame, as shown in Alg.~\ref{alg:1}.
%Alg.~\ref{alg:1} details how we select the reward function parameters.

Position weights are calculated using the equation:
\begin{equation}
\omega^i_p = K_p \frac{d_{\min}}{d_{t_{\min}}^{ij_{\min}}}.
\end{equation}
The angle and control weights all have the same value $\omega_{\alpha}^i = K_{\alpha}, ~ \gain^i_a = K_{a}$.
We set the contact weights $\gain^i_c$ to $K_c$ for all sensors that should be in contact. This can be done by asking participants where they feel the pressure during interactions. Alternatively, one could use the method from \cite{knoop2017handshakiness}, which simply applies color to the target hand and measures contact area from paint marks. 

To train the policy, we need to set just six weights in the reward function ($K_p, K_{\alpha}, K_c, K_{a}, K_{p I}, K_{\alpha I} $). In all our experiments, $K_{a}$ is set to 1, while $K_c$ is roughly set to $\frac{N_{o}}{5}$, where $N_{o}$ is the number of sensors that should be in contact.



%Weights for contact reward are set either to 0 or to $K_c$. The contact weights cannot be determined from motion capture data. 

%2 options:

%1)We put contact weights to $K_c$ to all sensors that are in contact. This can be done by simply asking users where do they feel the pressure, or if it is not easy to determine this, one could use method from ...

%2)We put contact weights to $K_c$ only on one contact sensor per finger. We can determine contact points on human hand simply by asking users where do they feel the pressure on the palm, or we can use method from... In human hand interaction finger can be pressured on multiple points, so we use man pressure point to determine which sensor to activate. For palm ....  


%First, we compute distances between the position features of both hands at each timestep $d^t_{ij}$, where $t$ is the timestep index, and $i=1..6$ and $j=1..6$ are the indexes of hand features on the actor and target hand respectively. Secondly, we find the minimum from calculated distances $d_{\min}= \min d^t_{ij}$, the respective time index $t_{\min}= \arg\min d^t_{ij}$ and the target hand feature index $j_{\min}= \arg\min d^t_{ij}$. When the distance is smallest, we can assume that hands are interacting. Goal joint angles are taken directly from actor hand joint angles at timestep $t_{\min}$. To compute goal positions, we memorize positions of the actor hand features $p^{j_{\min}}_i$ in the reference frame of target feature $j_{\min}$. 
%To compute goal positions, we simply add the memorized position to the current target hand feature position $p^g_i = p^j + R^j p^{j_{\min}}_i$, where $R^j$ is a rotation matrix of the target feature reference frame. The reward function is defined in a goal-centric way, which means that we can freely position the target hand in our simulation and calculate the reward function based on the new hand position. Finally, we compute reward weights as follows:
%\begin{align}
%& \omega^p_i = K_p \frac{d_{\min}}{d^{t_{\min}}_{ij_{\min}}} \\
%& \omega^{\alpha}_i = K_{\alpha}.
%\end{align}
%All angle weights are the same, while  position weights depend on the distance to the closest target feature. This way we just need to set two parameters for each interaction. \Stefan{(comment: maybe we can give this parameters)}  

\subsection{Training} 
\label{sec:training_alg}

To train the policy, we first need to position the target hand. For a single training episode, the target hand stays fixed. Although we train the policy with a static hand, we experimentally show that our policy generalizes to moving hands (cf. \ref{sec:policy_eval}). The joint angles of the target hand are set according to the joints of the human target hand at a timestep which occurs prior to the interaction timestep $t_{\min}$. This ensures that the target hand is not closed, thus allowing the robot to interact. Our reward function is defined in a goal centric way. This enables randomization of the target hand position, performed at the beginning of each episode. 
%\Sammy{We keep the target hand in the range of the agent hand.} 
To calculate the reward function parameters, we pick an interaction sequence uniformly at random.

%\Stefan{(Sammy comment: I would kill this next sentence and rephrase the sentence before to say that the joint angles are set at the time before the interaction happens instead of talking about a half second offset.)}

%The final state reward function is often enough to complete the interaction, i.e., to reach the final pose. However, the most direct trajectory often does not look natural. For example, in the case of a hand clap, the agent would simply position its hand on the target hand, omitting the characteristic clapping motion entirely. 
%We overcome this issue by adding an imitation reward. As shown in Sec.~\ref{sec:imitation_eval}, imitation reward significantly improves that the hand motion is perceived as natural. 
%However, when starting pose is far away from the demonstration trajectory, we sometimes observe non-smooth motions, which is a main drawback of our method. We evaluate these examples also in Sec.~\ref{sec:imitation_eval}. 

%A main drawback of our method, is that we observed non-smooth motions when starting pose is far away from the human demonstration trajectory. 
%The reason for non-smooth behavior is that there is no guidance to the demonstration trajectory. 


%However, this is not ideal for policy training, since the policy should work for any initial pose. \OH{How do we overcome this problem. If we don't do anything I'd rather remove these sentences.}

%Additionally, positioning the robot hand might not be feasible because of different configurations of the human and robot arms.

%Training with imitation cost assumes that the robot hand is positioned on the initial trajectory pose. 

%Imitation reward enforces the robot hand to follow the trajectory of the robot hand. However, positioning hand always at the beginning of the sequence is not practical from two reasons. First, the position might not be reachable due to different configurations of the human and robot arms. Second, this enforces that the hand starts from the same relative distance wrt. target hand, which might not be the case in the test case i.e., the robot hand should be able to execute interaction from any pose.   

We randomize the robot hand position additionally to target hand randomization. For imitation reward to be effective, the robot hand should be positioned in the same configuration as the human hand at the start of the imitation trajectory. Thus, we position the robot wrist to the position of the human wrist at timestep $t_s$, augmented with random Gaussian noise. The timestep $t_s$ is selected uniformly at random from a set $\{t_k \vert k=1 .. (t_{\min} - t_{\mathrm{off}})\}$. We use a small offset $t_{\mathrm{off}}$ because hands can collide in the last part of the trajectory. If this position is not reachable, we start from the closest reachable position. Contrary to \cite{peng2018deepmimic}, we cannot position the agent exactly in the human pose because of the configuration differences of the human and robot arms. Furthermore, our task is driven by a goal pose, which means that starting only from demonstration trajectories, as in \cite{peng2018deepmimic}, will result in poor generalization. After each $N_e$ steps, we update the network using the DRL algorithm described in Sec.~\ref{sec:drl}.

\subsection{Data Collection}

To collect data, we use the OptiTrack motion capture system. Each participant is equipped with markers as shown in Fig. \ref{fig:system}. We only track the right hand of each participant. 
Hand tracking is prone to marker mislabeling, with fingertip markers being most problematic. We use active markers, which can be uniquely identified by their blinking pattern, on the fingertips.
The OptriTrack software fits a model of the human hand to the markers, providing the position of each link and joint angle of the human hand. For each interaction, we recorded five demonstrations. We will release the dataset and simulation environment for further research (\href{https://ait.ethz.ch/projects/2019/DRL-handshake/}{https://ait.ethz.ch/projects/2019/DRL-handshake/}).
%\footnote{\href{https://ait.ethz.ch/projects/2019/DRL-handshake/}{https://ait.ethz.ch/projects/2019/DRL-handshake/}}.

%\oh{say that we will release data and environment for further research (if not say elsewhere)}

%In each demonstration, the first participant requests an interaction, while the second participant executes the interaction. The participants always put hands back to the rest pose and than execute the actions sequentially.

\begin{figure}
\centering
	\includegraphics[width= 0.60 \linewidth]{figures/system_2.png}
	\caption{\small{Participants wear 5 active markers on the fingertips and 6 passive markers on the palm and forearm of the right hand.}}
	\label{fig:system}
\end{figure}

%For each interaction, we recorded five demonstrations. In each demonstration, the first participant requests an interaction, while the second participant executes the interaction. 
%During data collection, the participants need to always put their hands back to the rest pose, then the first participant is requesting an interaction, and only then the second participant starts to act.


==> RAL_handshake (copy)/sec/05_results.tex <==
% !TEX root = ../paper.tex

\section{Results}

We conducted experiments in simulation to evaluate our method. We extensively test our policy on three different hand interactions: handshake, hand clap, and E.T. greeting (e.g. index finger touching), see Fig. \ref{fig:experiment_1_poses}. These three interactions are diverse: the handshake requires grasping of the target hand in a specific way, the hand clap has a characteristic motion prior to contact, while the E.T. greeting requires precise positioning of the index finger. 

\subsection{Ablation Study on Reward Function}
\label{sec:abl_study}

\begin{figure}
\centering
	\includegraphics[width=.95\linewidth]{figures/final_cost_comparison_new.png}
	\caption{\small{Final poses of the hands for different hand interactions.}}
	\label{fig:experiment_1_poses}
\end{figure}

In a first experiment, we intend to show the influence of the different parts of our reward function on the resulting control policy.
For this, we do an ablation study on our reward function.
We compare the full final state reward $\reward_F(\state{t}, \action{t})$ with two baselines. Baseline 1 uses only the relative position of the palm instead of the fingertips as a goal position feature, while keeping angle, contact and input reward the same. In Baseline 2, we remove the contact reward from the reward function. Furthermore, we examine the influence of adding the imitation reward to the final state reward.  
%We measure the success rate after each training epoch. 
%The success rate is estimated from the resulting contact profile on the hand. 

 
%We compare the trained policy with two baselines. The first baseline uses only the relative position of the palm as target position, while keeping angle, contact and input reward the same. This baseline is introduced to show the importance of the selected position features. The second baseline uses the proposed reward function without contact cost. This baseline is introduced to show importance of the contact cost. 

\begin{figure*}
\centering
	\includegraphics[width=0.98\linewidth]{figures/experiment_1_squeeze.png}
	\vspace{-0.2cm}
	\caption{\small{Baseline comparison. We measure the success rate of the policy every five epochs. Success is estimated from the contact profile on the hand. We show average results from 5 random seeds with the standard error indicated by the shaded area.}}
	\label{fig:experiment_1_fig}
	\vspace{-0.3cm}
\end{figure*}


Our final state reward function shows overall better performance than both baselines (c.f. Fig.~\ref{fig:experiment_1_fig}). The influence of the position reward can be seen by comparing Baseline 2 to Baseline 1 for handshake and E.T. interactions. Although both baselines have low success rates, Baseline 2 results in final configurations closer to the desired ones as shown in Fig.~\ref{fig:experiment_1_poses}. Adding contact reward to Baseline 2, i.e. using our reward function, removes these errors. The importance of the contact reward can be also seen in Fig.~\ref{fig:experiment_1_fig} in case of the hand clap. Since precise positioning is less important here, Baseline 1 achieves high success rate because of the contact reward. After adding the imitation reward, we observe that the success rates do not significantly change.

%\Stefan{Moreover, we noticed that the angle reward does not influence success rates, but creates visually more pleasing results by reaching desired final poses.}

%After adding imitation reward, we observe that the success rates for the handshake and E.T., although showing slower convergence, do not significantly change. For the hand clap, however, we see that the success rate is slightly lower. We believe that this is due to the problem of finding the balance between a reward that guides to the final position and the imitation reward that guides the hand off the direct trajectory.

%Importance of the contact reward can be seen by comparing full reward to Baseline 2 on Fig.~\ref{fig:experiment_1_poses} and on hand clap example on Fig~\ref{fig:experiment_1_fig}. 

%For the hand clap, we can see the importance of the contact reward. Both reward functions with contact reward achieve almost the same success rate, since precise positioning is less important here. Baseline 2 achieves low success rate scores, since it is not guided by the contact reward. However, final poses achieved with this reward are closer to desired ones, as shown in Fig.~\ref{fig:experiment_1_poses}. Absence of contact reward results in failure cases which are close in position but miss desired contacts (E.T. interaction) or reach unnatural hand positions (handshake). Moreover, we noticed that the angle reward does not influence success rates, but creates visually more pleasing results by reaching desired final poses.


%Our final state reward function shows overall better performance than both baselines (c.f. Fig.~\ref{fig:experiment_1_fig}). For the hand clap, we can see the importance of the contact reward. Both reward functions with contact reward achieve almost the same success rate, since precise positioning is less important here. Baseline 2 achieves low success rate scores, since it is not guided by contact reward. Absence of contact reward results in failure cases which are close in position but miss desired contacts (E.T. and hand clap) and also reach unnatural hand positions (handshake). Moreover, we noticed that the angle reward does not influence success rates, but creates visually more pleasing results by reaching desired final poses.\\
%After adding imitation reward, we observe that the success rates for the handshake and E.T., although showing slower convergence, do not significantly change. For the hand clap, however, we see that the success rate is slightly lower. We believe that this is due to the problem of finding the balance between a reward that guides to the final position and the imitation reward that guides the hand off the direct trajectory.

%is less important for this interaction.

%Without the contact reward, contact may not be achieved, as in the case of E.T. interaction, or hand can end up in unnatural position, as in the case of a handshake. 

% Results are shown in Fig. \ref{fig:experiment_1_fig}. As can be seen, the full final state reward achieves significantly lower errors on contact goals for the handshake and E.T. motion compared to both baselines. This indicates that both contact reward as well as all position features are required to successfully execute these interactions in terms of contacts that occur when humans execute these interactions. For the handclap, the difference is not as significant. This behavior can be explained with the high weight that needs to be on the angle reward in order to keep the fingers in a clapping position, while the goal of each finger being at the exact target position is not as important. Therefore, a general guiding position feature such as the palm in baseline 2 can achieve similar results for the hand clap as when using all position features. 


\subsection{Evaluation of Imitation Training}
\label{sec:imitation_eval}
To qualitatively assess the impact of the imitation reward, we conduct a large-scale user study ($N=116$). We present 11 video sequences of policy outputs with and without imitation reward side-by-side . We keep the initial conditions for each sequence-pair the same and randomly assign videos to the left or right. The participants state which video is perceived as more natural on a forced alternative choice 5-point scale. The five responses are: "Left sequence looks much more natural", "Left sequence looks more natural", "Both the same", "Right sequence looks more natural", "Right sequence looks much more natural".


%Keeping the initial conditions constant, we recorded two videos generated by policies with and without imitation reward. We then place the videos side-by-side and randomly assign them to the left or right. The users \Sammy{(I don't know what you want to say exactly here)} had forced alternative choice to define which video looks more natural. The five responses are: "Left sequence looks much more natural", "Left sequence looks more natural", "Both the same", "Right sequence looks more natural", "Right sequence looks much more natural". Each participant had to compare 11 videos. 

%\Sammy{(My suggestion of how to rephrase the paragraph before: 
%To evaluate the improvement of policies with imitation reward, we conducted a large-scale user study with 116 participants. The study is composed of 11 side-by-side video sequences of policies with and without imitation reward. We keep the initial conditions for each sequence-pair the same and only randomize the placement to avoid repetition bias. The users are asked to choose which interaction is perceived as more natural, with the possible answers being: "Left sequence looks much more natural", "Left sequence looks more natural", "Both the same", "Right sequence looks more natural", "Right sequence looks much more natural".)}

\begin{figure}
\centering
	\includegraphics[width=.95\linewidth]{figures/imitation_qual_clap.png}
	\caption{\small{Imitation reward. The policy trained with imitation reward produces a characteristic motion prior to the hand clap.}}
	\label{fig:experiment_2_qual_clap}
\end{figure}

%\begin{figure}
%\centering
%	\includegraphics[width=.95\linewidth]{figures/imitation_qual_shake.png}
%	\caption{\small{Imitation vs no imitation handshake.}}
%	\label{fig:experiment_2_qual_shake}
%\end{figure}

Assuming equidistant intervals, we mapped user responses onto a scale from -2 to 2, where positive values mean that the user prefers the policy generated with imitation reward and vice versa. The imitation policy can generate non-smooth motions when the starting pose is far away from the recorded human trajectory. To evaluate these examples, we compare two sequences including obvious non-smooth motions.

\begin{table}
\centering
\caption{User Study results of people voting on 5 point scale from -2 (no imitation) to 2 (imitation) looking much more natural}
\vspace{-6pt}
\resizebox{\columnwidth}{!}{
\begin{tabular}{| c | c | c | c | c | c | c |}
\hline
Score & $-2$ & $-1$ & $0$ & $1$ & $2$ & mean \\
\hline
Handshake & $4.9\%$ & $26.2\%$ & $15.2\%$ & $\mathbf{45.1\%}$ & $8.6\%$ & $0.26$ \\
\hline
Hand clap & $0.0\%$ & $2.3\%$ & $3.4\%$ & $41.9\%$ & $\mathbf{52.3\%}$ & $1.44$ \\
\hline
E.T. & $3.4\%$ & $17.2\%$ & $\mathbf{54.3\%}$ & $19.0\%$ & $6.0\%$ & $0.07$ \\
\hline
Handshake non-smooth & $23.3\%$ & $\mathbf{43.1\%}$ & $12.9\%$ & $15.5\%$ & $5.1\%$ & $-0.64$ \\
\hline
Hand clap non-smooth & $0.8\%$ & $7.0\%$ & $12.9\%$ & $\mathbf{49.1\%}$ & $30.2\%$ & $1.0$ \\
\hline
\end{tabular}\label{tbl:policies_compare}
}
\vspace{-14pt}
\end{table}


Generally speaking, participants favor policies generated with imitation reward (c.f. Table \ref{tbl:policies_compare}). For hand claps, the differences are easy to spot (see Fig.~\ref{fig:experiment_2_qual_clap}). Hence, human raters strongly prefer the imitation based policy. For the handshake, the differences are harder to see, resulting in significant amount of participants selecting "Both the same" ($15.2\%$). However, the majority of the participants still prefer the imitation based policy. 
For the E.T. interactions, there are no observable differences. Thus, the majority of participants answered with "Both the same" ($54.3\%$).
For non-smooth handshakes, the results indicate that participants prefer smooth motions. However, for non-smooth hand claps, participants prefer imitation features, although the mean score is lower than in the case of smooth hand claps.

%\oh{use plot as in Christoph's paper? Would safe space} \oh{make 'winning' entry bold}.


%The results in Table \ref{tbl:policies_compare} show that participants strongly favor imitation based policy. For handshake, the differences are harder to see. What happens is that without imitation robot hand readjusts position after grabbing the hand. On average, participants favor policy  with imitation. 


%The results in Table \ref{tbl:policies_compare} show that users are strongly in favor of the imitation policy for the hand clap, where the difference is easy to spot. An example of an imitation policy compared to a non-imitation policy is shown in Fig.~\ref{fig:experiment_2_qual_clap}.
%The handshake policies are harder to distinguish, which is why a significant amount of participants select "Both the same" ($15.2\%$). On average, however, more participants favor the policy with imitation. For the E.T. interactions, there are no observable differences. Thus, the majority of participants answered with "Both the same" ($54.3\%$). 
%For non-smooth examples, as in the case of a handshake where imitation differences are hard to spot, user study shows that participants prefer smooth motions. However, for non-smooth hand clap, participants prefer imitation features, although mean score is lower than in case of smooth hand claps. 

%\Sammy{(comment: I would rephrase the whole following paragraph, to be a bit more on point)}
 
% In terms of qualitative evaluation, we provide an example in Fig \ref{fig:experiment_2_qual_clap}. When we add imitation cost, there is a noticeable difference in the approaching trajectory for some interactions. E.g., for the handclap, we achieve the characteristic clapping motion instead of a trajectory that goes straight to the final pose. For the handshake, we notice a difference in some cases, specifically when the robot slides up on the target hand to reach the final pose without imitation, but has a better approaching angle with imitation. There is no visible difference in the E.T. motion, mainly since the approaching direction in the human demonstration data goes straight from the rest pose to the final pose.

%\begin{figure}
%\centering
%	\includegraphics[width=.95\linewidth]{figures/user_study.png}
%	\caption{\small{User study.}}
%	\label{fig:experiment_2_user_study}
%\end{figure}  

\subsection{Policy Evaluations}
\label{sec:policy_eval}

To evaluate the robustness of policies created with our method, we test the reaction to perturbations in orientation and velocity of the target hand. During training, we only randomize the position of the target hand, while the orientation stays the same. We position the target hand in the reachable workspace of the agent and measure the success rate, while changing the yaw and pitch angles of the target hand. In a realistic scenario, the human hand will not be perfectly still. Furthermore, the human can react when the contact is imminent by closing the hand or approaching the agent hand. Thus, we conduct a second experiment where the target hand is moving at constant speed, changing the direction at random every half second (see Fig.~\ref{fig:robustnes}).

\begin{figure}
\centering
	\includegraphics[width=.95\linewidth]{figures/robustnes_new_2.png}
	\caption{\small{Robustness experiments. Top: The average success rate for different target hand angles (the color bar shows the success rate). Down: The average success rate for different hand velocities. }}
	\label{fig:robustnes}
\end{figure}


The experiments indicate that our method is robust to perturbations in orientation and velocity of the target hand. This shows that our reward function generates policies that generalize well to unseen scenarios. 
%\Sammy{This is most likely due to the goal centric definition of our reward function.} 
We also tested our policy with changing configurations of the target hand, i.e., closing fingers in a handshake policy, and did not observe any major changes. Demonstrations of these experiments can be seen in the accompanying video (\href{https://youtu.be/ZSgEqyltaN4}{https://youtu.be/ZSgEqyltaN4}).


%\subsection{Experiments with User in Simulation}

==> RAL_handshake (copy)/sec/06_discussion.tex <==
% !TEX root = ../paper.tex

\section{Discussion and Conclusion}

Control of dexterous humanoid hands is a challenging problem, especially when it involves contact dynamics. 
%We address the problem of achieving natural human hand interactions using a humanoid hand robot. 
In this paper, we demonstrate that a single parametrized reward function can be used for different hand interactions. 
%to achieve multiple goals, including desired contact patterns. 
To define parameters of the reward function, we use a simple algorithm to extract parameters from motion capture data. 
%We augment the reward function with an imitation reward in order to produce more natural looking trajectories and validate it in a large-scale user study. 
We show that policies generated with our method produce more natural looking trajectories, and generalize well to different orientations and velocities of the target hand.
% We show that imitation reward produces more natural looking trajectories in a large-scale user study. Policies generated with our method generalize well to different orientations and velocities of the target hand.

Our results are shown only in simulation and with a static target hand as an initial step towards natural human-robot hand interactions. To achieve this level of performance on a real robot, transfer learning methods, such as the one suggested in \cite{openAI2018}, could be applied. 
%We hope that we can test our method on a real robot in future work.
We show that our policy reacts well to small velocity disturbances. However, humans can perform synchronous hand motions prior to interaction. This problem should be investigated in more detail. Our method only considers contacts, but we never investigated forces acting on the hand. \cite{knoop2017handshakiness} emphasizes the importance of forces applied during handshakes. According to our measurements, forces applied to the target hand are in the range of a normal handshake. 
Compliant behavior is important for hand interactions \cite{arns2017design}. However, evaluation of the robot hand compliance  is outside the scope of our work.    
%However, we did not investigate how the robot hand reacts to force disturbances. 
%Furthermore, some interactions, such as the handshake require compliant behavior of the robot \cite{arns2017design}. This needs further investigation and goes beyond the scope of this work.

%situations when small velocity disturbances are applied to the target hand

This paper shows how natural human-robot hand interaction can be learned using DRL. To the best of our knowledge, this is the first paper that uses a dexterous humanoid hand for human-robot hand interactions. This opens up the possibility to achieve natural hand interactions on a real humanoid robot.

%Furthermore, we investigated the possibility of achieving different hand interactions using human demonstrations.


==> RAL_handshake (copy)/sec/07_conclusion.tex <==
\section{Conclusion}

==> sec/07_conclusion.tex <==
\section{Conclusion}
